The Potential of the ILC for Discovering New Particles

This paper addresses the question of whether the International Linear Collider has the capability of discovering new particles that have not already been discovered at the CERN Large Hadron Collider. We summarize the various paths to discovery offered by the ILC, and discuss them in the context of three different scenarios: 1. LHC does not discover any new particles, 2. LHC discovers some new low mass states and 3. LHC discovers new heavy particles. We will show that in each case, ILC plays a critical role in discovery of new phenomena and in pushing forward the frontiers of high-energy physics as well as our understanding of the universe in a manner which is highly complementary to that of LHC. For the busy reader, a two-page executive summary is provided at the beginning of the document.

==> 06_bib-rp.tex <==
\bibliographystyle{apsrev}

\begin{thebibliography}{00}

\bibitem{Giudice:2008bi}
  G.~F.~Giudice,
  %``Naturally Speaking: The Naturalness Criterion and Physics at the LHC,''
  In *Kane, Gordon (ed.), Pierce, Aaron (ed.): Perspectives on LHC physics* 155-178
  [arXiv:0801.2562 [hep-ph]].
  %%CITATION = ARXIV:0801.2562;%%
  %70 citations counted in INSPIRE as of 14 Nov 2016

\bibitem{Wells:2004di}
  J.~D.~Wells,
  %``PeV-scale supersymmetry,''
  Phys.\ Rev.\ D {\bf 71} (2005) 015013
  doi:10.1103/PhysRevD.71.015013
  [hep-ph/0411041].
  %%CITATION = doi:10.1103/PhysRevD.71.015013;%%
  %222 citations counted in INSPIRE as of 20 Sep 2016

\bibitem{ArkaniHamed:2004fb}
  N.~Arkani-Hamed and S.~Dimopoulos,
  %``Supersymmetric unification without low energy supersymmetry and signatures for fine-tuning at the LHC,''
  JHEP {\bf 0506} (2005) 073
  doi:10.1088/1126-6708/2005/06/073
  [hep-th/0405159].
  %%CITATION = doi:10.1088/1126-6708/2005/06/073;%%
  %933 citations counted in INSPIRE as of 20 Sep 2016

\bibitem{Hall:2012zp}
  L.~J.~Hall, Y.~Nomura and S.~Shirai,
  %``Spread Supersymmetry with Wino LSP: Gluino and Dark Matter Signals,''
  JHEP {\bf 1301} (2013) 036
  doi:10.1007/JHEP01(2013)036
  [arXiv:1210.2395 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP01(2013)036;%%
  %96 citations counted in INSPIRE as of 20 Sep 2016

\bibitem{Acharya:2008zi}
  B.~S.~Acharya, K.~Bobkov, G.~L.~Kane, J.~Shao and P.~Kumar,
  %``The G(2)-MSSM: An M Theory motivated model of Particle Physics,''
  Phys.\ Rev.\ D {\bf 78} (2008) 065038
  doi:10.1103/PhysRevD.78.065038
  [arXiv:0801.0478 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.78.065038;%%
  %116 citations counted in INSPIRE as of 20 Sep 2016

\bibitem{Ibe:2012hu}
  M.~Ibe, S.~Matsumoto and T.~T.~Yanagida,
  %``Pure Gravity Mediation with m_{3/2} = 10-100TeV,''
  Phys.\ Rev.\ D {\bf 85} (2012) 095011
  doi:10.1103/PhysRevD.85.095011
  [arXiv:1202.2253 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.85.095011;%%
  %144 citations counted in INSPIRE as of 20 Sep 2016

\bibitem{Berggren:2013vfa}
  M.~Berggren, F.~Br\"ummer, J.~List, G.~Moortgat-Pick, T.~Robens, K.~Rolbiecki and H.~Sert,
  %``Tackling light higgsinos at the ILC,''
  Eur.\ Phys.\ J.\ C {\bf 73} (2013) no.12,  2660
  doi:10.1140/epjc/s10052-013-2660-y
  [arXiv:1307.3566 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-013-2660-y;%%
  %38 citations counted in INSPIRE as of 20 Sep 2016

\bibitem{Baltz:2006fm}
  E.~A.~Baltz, M.~Battaglia, M.~E.~Peskin and T.~Wizansky,
  %``Determination of dark matter properties at high-energy colliders,''
  Phys.\ Rev.\ D {\bf 74} (2006) 103521
  doi:10.1103/PhysRevD.74.103521
  [hep-ph/0602187].
  %%CITATION = doi:10.1103/PhysRevD.74.103521;%%
  %260 citations counted in INSPIRE as of 22 Nov 2016

\bibitem{Baer:2012cf}
  H.~Baer, V.~Barger, P.~Huang, D.~Mickelson, A.~Mustafayev and X.~Tata,
  %``Radiative natural supersymmetry: Reconciling electroweak fine-tuning and the Higgs boson mass,''
  Phys.\ Rev.\ D {\bf 87} (2013) no.11,  115028
  doi:10.1103/PhysRevD.87.115028
  [arXiv:1212.2655 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.87.115028;%%
  %111 citations counted in INSPIRE as of 20 Sep 2016

\bibitem{Baer:2015rja}
  H.~Baer, V.~Barger and M.~Savoy,
  %``Upper bounds on sparticle masses from naturalness or how to disprove weak scale supersymmetry,''
  Phys.\ Rev.\ D {\bf 93} (2016) no.3,  035016
  doi:10.1103/PhysRevD.93.035016
  [arXiv:1509.02929 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.93.035016;%%
  %14 citations counted in INSPIRE as of 20 Sep 2016

\bibitem{Baer:2013xua}
  H.~Baer, V.~Barger, P.~Huang, D.~Mickelson, A.~Mustafayev, W.~Sreethawong and X.~Tata,
  %``Radiatively-driven natural supersymmetry at the LHC,''
  JHEP {\bf 1312} (2013) 013
   Erratum: [JHEP {\bf 1506} (2015) 053]
  doi:10.1007/JHEP12(2013)013, 10.1007/JHEP06(2015)053
  [arXiv:1310.4858 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP12(2013)013, 10.1007/JHEP06(2015)053;%%
  %36 citations counted in INSPIRE as of 20 Sep 2016

\bibitem{Baer:2014yta}
  H.~Baer, V.~Barger, D.~Mickelson, A.~Mustafayev and X.~Tata,
  %``Physics at a Higgsino Factory,''
  JHEP {\bf 1406}, 172 (2014)
  doi:10.1007/JHEP06(2014)172
  [arXiv:1404.7510 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP06(2014)172;%%
  %23 citations counted in INSPIRE as of 26 Sep 2016

%\cite{Baer:2013cma}
\bibitem{Baer:2013cma}
  H.~Baer {\it et al.},
  %``The International Linear Collider Technical Design Report - Volume 2: Physics,''
  arXiv:1306.6352 [hep-ph].
  %%CITATION = ARXIV:1306.6352;%%
  %402 citations counted in INSPIRE as of 11 Oct 2016
  
  
 %\cite{Moortgat-Picka:2015yla}
\bibitem{Moortgat-Picka:2015yla}
  G.~Moortgat-Pick {\it et al.},
  %``Physics at the e+ e- Linear Collider,''
  Eur.\ Phys.\ J.\ C {\bf 75} (2015) no.8,  371
  doi:10.1140/epjc/s10052-015-3511-9
  [arXiv:1504.01726 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-015-3511-9;%%
  %48 citations counted in INSPIRE as of 11 Oct 2016
  
 %\cite{Djouadi:2007ik}
\bibitem{Djouadi:2007ik}
  G.~Aarons {\it et al.} [ILC Collaboration],
  %``International Linear Collider Reference Design Report Volume 2: Physics at the ILC,''
  arXiv:0709.1893 [hep-ph].
  %%CITATION = ARXIV:0709.1893;%%
  %335 citations counted in INSPIRE as of 11 Oct 2016
  
  %\cite{Asner:2013psa}
\bibitem{Asner:2013psa}
  D.~M.~Asner {\it et al.},
  %``ILC Higgs White Paper,''
  arXiv:1310.0763 [hep-ph].
  %%CITATION = ARXIV:1310.0763;%%
  %192 citations counted in INSPIRE as of 11 Oct 2016
  
  
  %\cite{Baer:2013vqa}
\bibitem{Baer:2013vqa}
  H.~Baer, M.~Berggren, J.~List, M.~M.~Nojiri, M.~Perelstein, A.~Pierce, W.~Porod and T.~Tanabe,
  %``Physics Case for the ILC Project: Perspective from Beyond the Standard Model,''
  arXiv:1307.5248 [hep-ph].
  %%CITATION = ARXIV:1307.5248;%%
  %19 citations counted in INSPIRE as of 11 Oct 2016

%\cite{Baak:2013fwa}
\bibitem{Baak:2013fwa}
  M.~Baak {\it et al.},
  %``Working Group Report: Precision Study of Electroweak Interactions,''
  arXiv:1310.6708 [hep-ph].
  %%CITATION = ARXIV:1310.6708;%%
  %77 citations counted in INSPIRE as of 11 Oct 2016

%\cite{Agashe:2013hma}
\bibitem{Agashe:2013hma}
  K.~Agashe {\it et al.} [Top Quark Working Group Collaboration],
  %``Working Group Report: Top Quark,''
  arXiv:1311.2028 [hep-ph].
  %%CITATION = ARXIV:1311.2028;%%
  %77 citations counted in INSPIRE as of 11 Oct 2016
  
  
  %\cite{Vos:2016til}
\bibitem{Vos:2016til}
  M.~Vos {\it et al.},
  %``Top physics at high-energy lepton colliders,''
  arXiv:1604.08122 [hep-ex].
  %%CITATION = ARXIV:1604.08122;%%
  %3 citations counted in INSPIRE as of 11 Oct 2016

 
%\cite{Fujii:2015jha}
\bibitem{Fujii:2015jha}
  K.~Fujii {\it et al.},
  ``Physics Case for the International Linear Collider,''
  arXiv:1506.05992 [hep-ex].
  %%CITATION = ARXIV:1506.05992;%%
  %62 citations counted in INSPIRE as of 11 Oct 2016
  
  
  %\cite{Barklow:2015tja}
\bibitem{Barklow:2015tja}
  T.~Barklow, J.~Brau, K.~Fujii, J.~Gao, J.~List, N.~Walker and K.~Yokoya,
  ``ILC Operating Scenarios,''
  arXiv:1506.07830 [hep-ex].
  %%CITATION = ARXIV:1506.07830;%%
  %46 citations counted in INSPIRE as of 11 Oct 2016
  
\bibitem{ICFAtoMEXT}  
  J.~Mnich {\it et al.}, ``The International Linear Collider: Comments on Scientific Significance
  and Technical Issues'' - in response to ``Summary of the ILC Advisory Panel's discussion to date (June 25 2015)'', December 15, 2015.

%%%% SH 



\bibitem{Degrassi:2012ry} 
  G.~Degrassi, S.~Di Vita, J.~Elias-Miro, J.~R.~Espinosa, G.~F.~Giudice, G.~Isidori and A.~Strumia,
  %``Higgs mass and vacuum stability in the Standard Model at NNLO,''
  JHEP {\bf 1208}, 098 (2012)
  doi:10.1007/JHEP08(2012)098
  [arXiv:1205.6497 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP08(2012)098;%%

%\cite{Richard:2014upa}
\bibitem{Richard:2014upa} 
  F.~Richard,
  %``Present and future constraints on top EW couplings,''
  arXiv:1403.2893 [hep-ph].
  %%CITATION = ARXIV:1403.2893;%%

\bibitem{Freitas:2013xga} 
  A.~Freitas, K.~Hagiwara, S.~Heinemeyer, P.~Langacker, K.~Moenig, M.~Tanabashi and G.~W.~Wilson,
  %``Exploring Quantum Physics at the ILC,''
  arXiv:1307.3962.
  %%CITATION = ARXIV:1307.3962;%%

\bibitem{Gupta:2013zza} 
  R.~S.~Gupta, H.~Rzehak and J.~D.~Wells,
  %``How well do we need to measure the Higgs boson mass and self-coupling?,''
  Phys.\ Rev.\ D {\bf 88}, 055024 (2013)
  doi:10.1103/PhysRevD.88.055024
  [arXiv:1305.6397 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.88.055024;%%

\bibitem{Osland:2009dp}
  P.~Osland, A.~A.~Pankov and A.~V.~Tsytrinov,
  %``Identification of extra neutral gauge bosons at the International Linear Collider,''
  Eur.\ Phys.\ J.\ C {\bf 67} (2010) 191
%  doi:10.1140/epjc/s10052-010-1272-z
  [arXiv:0912.2806 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-010-1272-z;%%

\bibitem{Godfrey:2005pm}
  S.~Godfrey, P.~Kalyniak and A.~Tomkins,
  %``Distinguishing between models with extra gauge bosons at the ILC,''
  hep-ph/0511335.
  %%CITATION = HEP-PH/0511335;%%

\bibitem{Godfrey:2000hc}
  S.~Godfrey, P.~Kalyniak, B.~Kamal and A.~Leike,
  %``Discovery and identification of extra gauge bosons in e+ e- ---> neutrino anti-neutrino gamma,''
  Phys.\ Rev.\ D {\bf 61} (2000) 113009
%  doi:10.1103/PhysRevD.61.113009
  [hep-ph/0001074].
  %%CITATION = doi:10.1103/PhysRevD.61.113009;%%

\bibitem{Baer:2016hfa}
  H.~Baer, V.~Barger, H.~Serce and X.~Tata,
  %``Natural generalized mirage mediation,''
  arXiv:1610.06205 [hep-ph].

\bibitem{Anderson:1999uia}
  G.~Anderson, H.~Baer, C.~h.~Chen and X.~Tata,
  %``The Reach of Fermilab Tevatron upgrades for SU(5) supergravity models with nonuniversal gaugino masses,''
  Phys.\ Rev.\ D {\bf 61} (2000) 095005
  doi:10.1103/PhysRevD.61.095005
  [hep-ph/9903370].

\bibitem{Moroi:1999zb}
  T.~Moroi and L.~Randall,
  %``Wino cold dark matter from anomaly mediated SUSY breaking,''
  Nucl.\ Phys.\ B {\bf 570} (2000) 455
  doi:10.1016/S0550-3213(99)00748-8
  [hep-ph/9906527].

\bibitem{Fan:2013faa}
  J.~Fan and M.~Reece,
  %``In Wino Veritas? Indirect Searches Shed Light on Neutralino Dark Matter,''
  JHEP {\bf 1310} (2013) 124
  doi:10.1007/JHEP10(2013)124
  [arXiv:1307.4400 [hep-ph]].

\bibitem{Cohen:2013ama}
  T.~Cohen, M.~Lisanti, A.~Pierce and T.~R.~Slatyer,
  %``Wino Dark Matter Under Siege,''
  JCAP {\bf 1310} (2013) 061
  doi:10.1088/1475-7516/2013/10/061
  [arXiv:1307.4082 [hep-ph]].

\bibitem{Murayama:1992dj}
  H.~Murayama, H.~Suzuki and T.~Yanagida,
  %``Radiative breaking of Peccei-Quinn symmetry at the intermediate mass scale,''
  Phys.\ Lett.\ B {\bf 291} (1992) 418.
  doi:10.1016/0370-2693(92)91397-R

\bibitem{Bae:2015rra}
  K.~J.~Bae, H.~Baer, A.~Lessa and H.~Serce,
  %``Mixed axion-wino dark matter,''
  Front.\ in Phys.\  {\bf 3} (2015) 49
  doi:10.3389/fphy.2015.00049
  [arXiv:1502.07198 [hep-ph]].

\bibitem{Bae:2014yta}
  K.~J.~Bae, H.~Baer and H.~Serce,
  %``Natural little hierarchy for SUSY from radiative breaking of the Peccei-Quinn symmetry,''
  Phys.\ Rev.\ D {\bf 91} (2015) no.1,  015003
  doi:10.1103/PhysRevD.91.015003
  [arXiv:1410.7500 [hep-ph]].

\bibitem{Bartels:2012ex}
  C.~Bartels, M.~Berggren and J.~List,
  %``Characterising WIMPs at a future $e^+e^-$ Linear Collider,''
  Eur.\ Phys.\ J.\ C {\bf 72} (2012) 2213
  doi:10.1140/epjc/s10052-012-2213-9
  [arXiv:1206.6639 [hep-ex]].

\bibitem{Baer:2016usl}
  H.~Baer, V.~Barger, M.~Savoy and X.~Tata,
  %``Multichannel assault on natural supersymmetry at the high luminosity LHC,''
  Phys.\ Rev.\ D {\bf 94} (2016) no.3,  035025
  doi:10.1103/PhysRevD.94.035025
  [arXiv:1604.07438 [hep-ph]].



%%%% SH end


%%%% Top Mass References - FS 

\bibitem{Seidel:2013sqa} 
  K.~Seidel, F.~Simon, M.~Tesar and S.~Poss,
  %``Top quark mass measurements at and above threshold at CLIC,''
  Eur.\ Phys.\ J.\ C {\bf 73}, 2530 (2013)
  [arXiv:1303.3758 [hep-ex]].
  %%CITATION = doi:10.1140/epjc/s10052-013-2530-7;%%
  
  \bibitem{Beneke:2015kwa} 
  M.~Beneke {\it et al.}, %Y.~Kiyo, P.~Marquard, A.~Penin, J.~Piclum and M.~Steinhauser,
%  ``Next-to-Next-to-Next-to-Leading Order QCD Prediction for the Top Antitop $S$-Wave Pair Production Cross Section Near Threshold in $e^+e^-$ Annihilation,''
  Phys.\ Rev.\ Lett.\  {\bf 115}, 192001 (2015)
 % doi:10.1103/PhysRevLett.115.192001
  [arXiv:1506.06864 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.115.192001;%%

\bibitem{Simon:2016htt} 
  F.~Simon,
  %``A First Look at the Impact of NNNLO Theory Uncertainties on Top Mass Measurements at the ILC,''
  arXiv:1603.04764 [hep-ex].
  %%CITATION = ARXIV:1603.04764;%%  
  
  \bibitem{Simon:2016pwp} 
  F.~Simon,
  %``Impact of Theory Uncertainties on the Precision of the Top Quark Mass in a Threshold Scan at Future e+e- Colliders,''
  arXiv:1611.03399 [hep-ex].
  %%CITATION = ARXIV:1611.03399;%%

\bibitem{Marquard:2015qpa} 
  P.~Marquard, A.~V.~Smirnov, V.~A.~Smirnov and M.~Steinhauser,
  %``Quark Mass Relations to Four-Loop Order in Perturbative QCD,''
  Phys.\ Rev.\ Lett.\  {\bf 114}, no. 14, 142002 (2015) 
  [arXiv:1502.01030 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.114.142002;%%
%%%% Top Mass References - FS end

%\cite{Fleper:2016frz}
\bibitem{Fleper:2016frz} 
  C.~Fleper, W.~Kilian, J.~Reuter and M.~Sekulla,
  %``Scattering of W and Z Bosons at High-Energy Lepton Colliders,''
  arXiv:1607.03030 [hep-ph].
  %%CITATION = ARXIV:1607.03030;%%
  
  
\bibitem{Baer:2001ia}
  H.~Baer and A.~Belyaev,
  %``Associated neutralino neutralino photon production at NLC,''
  eConf C {\bf 010630} (2001) P336
  [hep-ph/0111017].
  %%CITATION = HEP-PH/0111017;%%
  %9 citations counted in INSPIRE as of 14 Jun 2013

%\cite{Birkedal:2004xn}
\bibitem{Birkedal:2004xn}
  A.~Birkedal, K.~Matchev and M.~Perelstein,
  %``Dark matter at colliders: A Model independent approach,''
  Phys.\ Rev.\ D {\bf 70} (2004) 077701
  [hep-ph/0403004].
  %%CITATION = HEP-PH/0403004;%%
  %87 citations counted in INSPIRE as of 10 Jun 2013
  
%\cite{Dreiner:2012xm}
\bibitem{Dreiner:2012xm}
  H.~Dreiner, M.~Huck, M.~Kr\"amer, D.~Schmeier and J.~Tattersall,
  %``Illuminating Dark Matter at the ILC,''
  Phys.\ Rev.\ D {\bf 87} (2013) 075015
  [arXiv:1211.2254 [hep-ph]].
  %%CITATION = ARXIV:1211.2254;%%
  %4 citations counted in INSPIRE as of 01 Jun 2013
  
%\cite{Chae:2012bq}
\bibitem{Chae:2012bq}
  Y.~J.~Chae and M.~Perelstein,
  ``Dark Matter Search at a Linear Collider: Effective Operator Approach,''
  arXiv:1211.4008 [hep-ph].
  %%CITATION = ARXIV:1211.4008;%%
  %4 citations counted in INSPIRE as of 10 Jun 2013

\bibitem{bib:chaus}
  A.~Chaus, ``Searches for Dark Matter particules and development of a pixellized readout of the Time Projection Chamber for
the International Linear Collider (ILC),'' PhD thesis, 2014, Universit\'e Paris 11
\url{http://www.theses.fr/2014PA112300}.

\bibitem{bib:habermehl}
 M.~Habermehl {\it et al.}, ``,'' proceedings ICHEP 2016.

%\cite{List:2013dga}
\bibitem{List:2013dga}
  B.~Vormwald and J.~List,
  %``Bilinear $R$ parity violation at the ILC: neutrino physics at colliders,''
  Eur.\ Phys.\ J.\ C {\bf 74} (2014) 2720
  doi:10.1140/epjc/s10052-014-2720-y
  [arXiv:1307.4074 [hep-ex]].
  %%CITATION = doi:10.1140/epjc/s10052-014-2720-y;%%
  %11 citations counted in INSPIRE as of 14 Nov 2016
  
  
\bibitem{bib:ATLAS_bRPV}
ATLAS Collaboration, ``Search for supersymmetry at sqrts=7~TeV~in final states with large jet multiplicity, missing transverse momentum and one isolated lepton with the ATLAS detector,'' ATLAS-CONF-2012-140, \url{http://cds.cern.ch/record/1483511}.

\bibitem{Panico:2015jxa}
  G.~Panico and A.~Wulzer,
  %``The Composite Nambu-Goldstone Higgs,''
  Lect.\ Notes Phys.\  {\bf 913} (2016) pp.1
  doi:10.1007/978-3-319-22617-0
  [arXiv:1506.01961 [hep-ph]].
  %%CITATION = doi:10.1007/978-3-319-22617-0;%%
  %84 citations counted in INSPIRE as of 14 Nov 2016
  
\bibitem{Csaki:2008zd}
  C.~Csaki, A.~Falkowski and A.~Weiler,
  %``The Flavor of the Composite Pseudo-Goldstone Higgs,''
  JHEP {\bf 0809} (2008) 008
  doi:10.1088/1126-6708/2008/09/008
  [arXiv:0804.1954 [hep-ph]].
  %%CITATION = doi:10.1088/1126-6708/2008/09/008;%%

\bibitem{Falkowski:2007hz}
  A.~Falkowski,
  %``Pseudo-goldstone Higgs production via gluon fusion,''
  Phys.\ Rev.\ D {\bf 77} (2008) 055018
  doi:10.1103/PhysRevD.77.055018
  [arXiv:0711.0828 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.77.055018;%%  
  
\bibitem{LHCHiggsCrossSectionWorkingGroup:2012nn}
  A.~David {\it et al.} [LHC Higgs Cross Section Working Group Collaboration],
  %``LHC HXSWG interim recommendations to explore the coupling structure of a Higgs-like particle,''
  arXiv:1209.0040 [hep-ph].
  %%CITATION = ARXIV:1209.0040;%%  
  
\bibitem{Ellis:1975ap}
  J.~R.~Ellis, M.~K.~Gaillard and D.~V.~Nanopoulos,
  %``A Phenomenological Profile of the Higgs Boson,''
  Nucl.\ Phys.\ B {\bf 106} (1976) 292.
  doi:10.1016/0550-3213(76)90382-5
  %%CITATION = doi:10.1016/0550-3213(76)90382-5;%%
  
  \bibitem{Shifman:1979eb}
  M.~A.~Shifman, A.~I.~Vainshtein, M.~B.~Voloshin and V.~I.~Zakharov,
  %``Low-Energy Theorems for Higgs Boson Couplings to Photons,''
  Sov.\ J.\ Nucl.\ Phys.\  {\bf 30} (1979) 711
   [Yad.\ Fiz.\  {\bf 30} (1979) 1368].
  %%CITATION = SJNCA,30,711;%%  

  
\bibitem{Azatov:2016xik}
  A.~Azatov, C.~Grojean, A.~Paul and E.~Salvioni,
  %``Resolving gluon fusion loops at current and future hadron colliders,''
  JHEP {\bf 1609} (2016) 123
  doi:10.1007/JHEP09(2016)123
  [arXiv:1608.00977 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP09(2016)123;%%
  
    \bibitem{Azatov:2015oxa}
  A.~Azatov, R.~Contino, G.~Panico and M.~Son,
  %``Effective field theory analysis of double Higgs boson production via gluon fusion,''
  Phys.\ Rev.\ D {\bf 92} (2015) no.3,  035001
  doi:10.1103/PhysRevD.92.035001
  [arXiv:1502.00539 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.035001;%%
    
\bibitem{Agashe:2004rs}
  K.~Agashe, R.~Contino and A.~Pomarol,
  %``The Minimal composite Higgs model,''
  Nucl.\ Phys.\ B {\bf 719} (2005) 165
  doi:10.1016/j.nuclphysb.2005.04.035
  [hep-ph/0412089].
  %%CITATION = doi:10.1016/j.nuclphysb.2005.04.035;%%
  
  \bibitem{Contino:2006qr}
  R.~Contino, L.~Da Rold and A.~Pomarol,
  %``Light custodians in natural composite Higgs models,''
  Phys.\ Rev.\ D {\bf 75} (2007) 055014
  doi:10.1103/PhysRevD.75.055014
  [hep-ph/0612048].
  %%CITATION = doi:10.1103/PhysRevD.75.055014;%%
  
  \bibitem{Pappadopulo:2013vca}
  D.~Pappadopulo, A.~Thamm and R.~Torre,
  %``A minimally tuned composite Higgs model from an extra dimension,''
  JHEP {\bf 1307} (2013) 058
  doi:10.1007/JHEP07(2013)058
  [arXiv:1303.3062 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP07(2013)058;%%
  
  \bibitem{Low:2009di}
  I.~Low, R.~Rattazzi and A.~Vichi,
  %``Theoretical Constraints on the Higgs Effective Couplings,''
  JHEP {\bf 1004} (2010) 126
  doi:10.1007/JHEP04(2010)126
  [arXiv:0907.5413 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP04(2010)126;%%
  
  \bibitem{deBlas:2016ojx}
  J.~de Blas, M.~Ciuchini, E.~Franco, S.~Mishima, M.~Pierini, L.~Reina and L.~Silvestrini,
  %``Electroweak precision observables and Higgs-boson signal strengths in the Standard Model and beyond: present and future,''
  arXiv:1608.01509 [hep-ph].
  %%CITATION = ARXIV:1608.01509;%%    
    
\bibitem{Azatov:2014jga}
  A.~Azatov, C.~Grojean, A.~Paul and E.~Salvioni,
  %``Taming the off-shell Higgs boson,''
  Zh.\ Eksp.\ Teor.\ Fiz.\  {\bf 147} (2015) 410
   [J.\ Exp.\ Theor.\ Phys.\  {\bf 120} (2015) 354]
  doi:10.1134/S1063776115030140, 10.7868/S0044451015030039
  [arXiv:1406.6338 [hep-ph]].
  %%CITATION = doi:10.1134/S1063776115030140, 10.7868/S0044451015030039;%%    

\bibitem{Grojean:2013qca}
  C.~Grojean, O.~Matsedonskyi and G.~Panico,
  %``Light top partners and precision physics,''
  JHEP {\bf 1310} (2013) 160
  doi:10.1007/JHEP10(2013)160
  [arXiv:1306.4655 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP10(2013)160;%%

\bibitem{Chacko:2005pe}
  Z.~Chacko, H.~S.~Goh and R.~Harnik,
  %``The Twin Higgs: Natural electroweak breaking from mirror symmetry,''
  Phys.\ Rev.\ Lett.\  {\bf 96} (2006) 231802
  doi:10.1103/PhysRevLett.96.231802
  [hep-ph/0506256].
  %%CITATION = doi:10.1103/PhysRevLett.96.231802;%%

\bibitem{Chacko:2005un}
  Z.~Chacko, H.~S.~Goh and R.~Harnik,
  %``A Twin Higgs model from left-right symmetry,''
  JHEP {\bf 0601} (2006) 108
  doi:10.1088/1126-6708/2006/01/108
  [hep-ph/0512088].
  %%CITATION = doi:10.1088/1126-6708/2006/01/108;%%

\bibitem{Craig:2015pha}
  N.~Craig, A.~Katz, M.~Strassler and R.~Sundrum,
  %``Naturalness in the Dark at the LHC,''
  JHEP {\bf 1507} (2015) 105
  doi:10.1007/JHEP07(2015)105
  [arXiv:1501.05310 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP07(2015)105;%%

\bibitem{Dimopoulos:1981zb}
S.~Dimopoulos and H.~Georgi, ``{Softly Broken Supersymmetry and SU(5) }'' {\em
  Nucl.Phys.} {\bf B193}  150.

\bibitem{Feng:1995zd}
  J.~L.~Feng, M.~E.~Peskin, H.~Murayama and X.~R.~Tata,
  %``Testing supersymmetry at the next linear collider,''
  Phys.\ Rev.\ D {\bf 52} (1995) 1418
  doi:10.1103/PhysRevD.52.1418
  [hep-ph/9502260].
  %%CITATION = doi:10.1103/PhysRevD.52.1418;%%


\bibitem{Berggren:2013vna}
M.~Berggren, ``{Simplified SUSY at the ILC }''
\href{http://arxiv.org/abs/1308.1461}{{\tt arXiv:1308.1461 [hep-ph]}}.
%%CITATION = ARXIV:1308.1461;%%.

\bibitem{Aad:2014vma}
{\bf ATLAS Collaboration}, G.~Aad {\em et al.}, ``{Search for direct production
  of charginos, neutralinos and sleptons in final states with two leptons and
  missing transverse momentum in $pp$ collisions at $\sqrt{s} =$ 8 TeV with the
  ATLAS detector }'' {\em JHEP} {\bf 1405}  071.

\bibitem{ATLAS:2013hta}
{\bf ATLAS Collaboration}, ``{Physics at a High-Luminosity LHC with ATLAS }''
\href{http://arxiv.org/abs/1307.7292}{{\tt arXiv:1307.7292 [hep-ex]}}.
%%CITATION = ARXIV:1307.7292;%%.

\bibitem{Heister:2002mn}
{\bf ALEPH Collaboration}, A.~Heister {\em et al.}, ``{Search for charginos
  nearly mass degenerate with the lightest neutralino in e+ e- collisions at
  center-of-mass energies up to 209-GeV }'' {\em Phys.Lett.} {\bf B533}
  223--236.

\bibitem{Abdallah:2003xe}
{\bf DELPHI Collaboration}, J.~Abdallah {\em et al.}, ``{Searches for
  supersymmetric particles in e+ e- collisions up to 208-GeV and interpretation
  of the results within the MSSM }'' {\em Eur.Phys.J.} {\bf C31}  421--479.

\bibitem{Abbiendi:2002vz}
{\bf OPAL Collaboration}, G.~Abbiendi {\em et al.}, ``{Search for nearly mass
  degenerate charginos and neutralinos at LEP }'' {\em Eur.Phys.J.} {\bf C29}
  479--489.

\bibitem{Kilian:2004pp} 
  W.~Kilian, D.~Rainwater and J.~Reuter,
  %``Pseudo-axions in little Higgs models,''
  Phys.\ Rev.\ D {\bf 71}, 015008 (2005)
  doi:10.1103/PhysRevD.71.015008
  [hep-ph/0411213].
  %%CITATION = doi:10.1103/PhysRevD.71.015008;%%

\bibitem{Ade:2015xua}                                                                                     
Planck Collaboration, P.~A.~R. Ade {\em et~al.},                                                          
{\em Planck 2015  results. XIII. Cosmological parameters},                                                
Astron.\ Astrophys.\  {\bf 594} (2016) A13                                                                
[\href{http://arxiv.org/abs/1502.01589}{{\ttfamily arXiv:1502.01589                                       
  [astro-ph.CO]}}].                                                                                       
%%CITATION = ARXIV:1502.01589;%%.                                                                         
                                                                                                          
%\cite{deVries:2015hva}                                                                                   
\bibitem{deVries:2015hva}                                                                                 
  K.~J.~de Vries {\it et al.},                                                                            
 {\em The pMSSM10 after LHC Run 1},                                                                       
  Eur.\ Phys.\ J.\ C {\bf 75} (2015) no.9,  422                                                           
  %%doi:10.1140/epjc/s10052-015-3599-y                                                                    
[\href{http://arxiv.org/abs/1504.03260}{{\ttfamily arXiv:1504.03260 [hep-ph]}}].                          
%%  [arXiv:1504.03260 [hep-ph]].                                                                          
  %%CITATION = doi:10.1140/epjc/s10052-015-3599-y;%%                                                      
  %40 citations counted in INSPIRE as of 09 Nov 2016                                                      
                                                                                                          
%%%microomegas:                                                                                           
\bibitem{Belanger:2006is}                                                                                 
G.~Belanger  {\it et al.},                                                                                
%% , F.~Boudjema, A.~Pukhov, and A.~Semenov,                                                              
 {\em MicrOMEGAs 2.0: A Program to calculate the relic density of dark matter in a generic model},        
  \href{http://dx.doi.org/10.1016/j.cpc.2006.11.008}{ Comput. Phys.                                       
  Commun. {\bfseries 176} (2007) 367--382},                                                               
  [\href{http://arxiv.org/abs/hep-ph/0607059}{{\ttfamily arXiv:hep-ph/0607059}}].                         
                                                                                                          
\bibitem{Lehtinen:2016qis}                                                                                
  S.~L.~Lehtinen, M.~Berggren and J.~List,                                                                
  {\em Dark matter relic density from observations of supersymmetry at the ILC},                          
\href{http://arxiv.org/abs/1602.08439}{{\ttfamily arXiv:1602.08439 [hep-ph]}}                             
%%  arXiv:1602.08439 [hep-ph].                                                                            
  %%CITATION = ARXIV:1602.08439;%%                                                                        
                                                                                                          
\bibitem{Baer:2013ula}                                                                                    
H.~Baer and J.~List,                                                                                      
{\em Post LHC8 SUSY benchmark points for ILC physics},                                                    
  \href{http://dx.doi.org/10.1103/PhysRevD.88.055004}{ Phys. Rev.                                         
  {\bfseries D88} (2013) 055004},                                                                         
[\href{http://arxiv.org/abs/1307.0782}{{\ttfamily arXiv:1307.0782 [hep-ph]}}].                            
%%CITATION = ARXIV:1307.0782;%%.                                                                          
                                                                                                          
%%% our note:                                                                                             
\bibitem{Berggren:2015qua}                                                                                
M.~Berggren  {\it et al.},                                                                                
%, A.~Cakir, D.~Kr{\"u}cker, J.~List, I.~A. Melzer-Pellmann, B.~S.                                        
%  Samani, C.~Seitz, and S.~Wayand,                                                                       
{\em Non-Simplified SUSY: Stau-Coannihilation  at LHC and ILC},                                           
  Eur.\ Phys.\ J.\ C {\bf 76} (2016) no.4,  183                                                           
[\href{http://arxiv.org/abs/1508.04383}{{\ttfamily arXiv:1508.04383 [hep-ph]}}].                          
%%CITATION = ARXIV:1508.04383;%%.                                                                         
                                                                                                          
\bibitem{Bechtle:2009em}                                                                                  
 P.~Bechtle  {\it et al.},                                                                                
%% , M.~Berggren, J.~List, P.~Schade, and O.~Stempel,                                                     
{\em Prospects for the study of the $\tilde{\tau}$-system in SPS1a' at the ILC},                          
   \href{http://dx.doi.org/10.1103/PhysRevD.82.055016}{ Phys. Rev.                                        
   {\bfseries D82} (2010) 055016},                                                                        
 [\href{http://arxiv.org/abs/0908.0876}{{\ttfamily arXiv:0908.0876 [hep-ex]}}].                           
%% %%CITATION = ARXIV:0908.0876;%%.                                                                       

%\cite{Potter:2015wsa}
\bibitem{Potter:2015wsa} 
  C.~T.~Potter,
  %``Natural NMSSM with a Light Singlet Higgs and Singlino LSP,''
  Eur.\ Phys.\ J.\ C {\bf 76}, no. 1, 44 (2016)
  doi:10.1140/epjc/s10052-015-3867-x
  [arXiv:1505.05554 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-015-3867-x;%%
  %10 citations counted in INSPIRE as of 16 Nov 2016

%\cite{Potter:2015wsa}
\bibitem{Potter:ECFALC2016} 
  C.~T.~Potter,
  ``The NMSSM Singlet at the ILC,''
  presented at ECFA-LC 2016.

%\cite{ArkaniHamed:2001nc}
\bibitem{ArkaniHamed:2001nc} 
  N.~Arkani-Hamed, A.~G.~Cohen and H.~Georgi,
  %``Electroweak symmetry breaking from dimensional deconstruction,''
  Phys.\ Lett.\ B {\bf 513}, 232 (2001)
  doi:10.1016/S0370-2693(01)00741-9
  [hep-ph/0105239].
  %%CITATION = doi:10.1016/S0370-2693(01)00741-9;%%

%\cite{ArkaniHamed:2002qx}
\bibitem{ArkaniHamed:2002qx} 
  N.~Arkani-Hamed, A.~G.~Cohen, E.~Katz, A.~E.~Nelson, T.~Gregoire and J.~G.~Wacker,
  %``The Minimal moose for a little Higgs,''
  JHEP {\bf 0208}, 021 (2002)
  doi:10.1088/1126-6708/2002/08/021
  [hep-ph/0206020].
  %%CITATION = doi:10.1088/1126-6708/2002/08/021;%%

%\cite{ArkaniHamed:2002qy}
\bibitem{ArkaniHamed:2002qy} 
  N.~Arkani-Hamed, A.~G.~Cohen, E.~Katz and A.~E.~Nelson,
  %``The Littlest Higgs,''
  JHEP {\bf 0207}, 034 (2002)
  doi:10.1088/1126-6708/2002/07/034
  [hep-ph/0206021].
  %%CITATION = doi:10.1088/1126-6708/2002/07/034;%%

%\cite{Schmaltz:2004de}
\bibitem{Schmaltz:2004de} 
  M.~Schmaltz,
  %``The Simplest little Higgs,''
  JHEP {\bf 0408}, 056 (2004)
  doi:10.1088/1126-6708/2004/08/056
  [hep-ph/0407143].
  %%CITATION = doi:10.1088/1126-6708/2004/08/056;%%
  
%\cite{BhupalDev:2007ftb}
\bibitem{BhupalDev:2007ftb}
  P.~S.~Bhupal Dev, A.~Djouadi, R.~M.~Godbole, M.~M.~Muhlleitner and S.~D.~Rindani,
  %``Determining the CP properties of the Higgs boson,''
  Phys.\ Rev.\ Lett.\  {\bf 100} (2008) 051801
  doi:10.1103/PhysRevLett.100.051801
  [arXiv:0707.2878 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.100.051801;%%
  %70 citations counted in INSPIRE as of 21 Nov 2016  


%\cite{Senaha:2013fva}
\bibitem{Senaha:2013fva}
  E.~Senaha,
  %``Overview of Electroweak Baryogenesis,''
  arXiv:1305.1563 [hep-ph].
  %%CITATION = ARXIV:1305.1563;%%
  %3 citations counted in INSPIRE as of 21 Nov 2016

%\cite{Hashino:2015nxa}
\bibitem{Hashino:2015nxa}
  K.~Hashino, S.~Kanemura and Y.~Orikasa,
  %``Discriminative phenomenological features of scale invariant models for electroweak symmetry breaking,''
  Phys.\ Lett.\ B {\bf 752} (2016) 217
  doi:10.1016/j.physletb.2015.11.044
  [arXiv:1508.03245 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2015.11.044;%%
  %10 citations counted in INSPIRE as of 21 Nov 2016

\bibitem{Tian:2013}
J.~Tian and K.~Fujii, "Study of Higgs self-coupling at the ILC 
based on the full detector simulation 
at $\sqrt{s}$ = 500 GeV and 1 TeV", 
LC-REP-2013-003.

\bibitem{Kurata:2013}
M.~Kurata {\it et al.}, "The Higgs self-coupling analysis 
using the events containing $H\to WW^*$ decay"
LC-REP-2013-025.

\bibitem{Duerig:2016}
C.~Duerig, "Measuring the Higgs Self-coupling at the International Linear Collider"
PhD Thesis.

\bibitem{Tian:2015}
J.~Tian and K.~Fujii, "ZHH cross section analysis", 
talk at the LCWS15, paper in preparation.

%\cite{McCullough:2013rea}
\bibitem{McCullough:2013rea}
  M.~McCullough,
  %``An Indirect Model-Dependent Probe of the Higgs Self-Coupling,''
  Phys.\ Rev.\ D {\bf 90} (2014) no.1,  015001
   Erratum: [Phys.\ Rev.\ D {\bf 92} (2015) no.3,  039903]
  doi:10.1103/PhysRevD.90.015001, 10.1103/PhysRevD.92.039903
  [arXiv:1312.3322 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.90.015001, 10.1103/PhysRevD.92.039903;%%
  %36 citations counted in INSPIRE as of 21 Nov 2016

\bibitem{Barklow:2016}
T.~Barklow, K.~Fujii, S.~Jung, M.~Peskin and J.~Tian and K.~Fujii, 
"Model-Independent Determination of the Triple Higgs Coupling at e+e- Colliders", 
paper in preparation.

%\cite{Aad:2015mxa}
\bibitem{Aad:2015mxa}
  G.~Aad {\it et al.} [ATLAS Collaboration],
  %``Study of the spin and parity of the Higgs boson in diboson decays with the ATLAS detector,''
  Eur.\ Phys.\ J.\ C {\bf 75} (2015) no.10,  476
   Erratum: [Eur.\ Phys.\ J.\ C {\bf 76} (2016) no.3,  152]
  doi:10.1140/epjc/s10052-015-3685-1, 10.1140/epjc/s10052-016-3934-y
  [arXiv:1506.05669 [hep-ex]].
  %%CITATION = doi:10.1140/epjc/s10052-015-3685-1, 10.1140/epjc/s10052-016-3934-y;%%
  %80 citations counted in INSPIRE as of 21 Nov 2016

%\cite{Khachatryan:2014kca}
\bibitem{Khachatryan:2014kca}
  V.~Khachatryan {\it et al.} [CMS Collaboration],
  %``Constraints on the spin-parity and anomalous HVV couplings of the Higgs boson in proton collisions at 7 and 8 TeV,''
  Phys.\ Rev.\ D {\bf 92} (2015) no.1,  012004
  doi:10.1103/PhysRevD.92.012004
  [arXiv:1411.3441 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevD.92.012004;%%
  %160 citations counted in INSPIRE as of 21 Nov 2016

%\cite{Grzadkowski:1995rx}
\bibitem{Grzadkowski:1995rx}
  B.~Grzadkowski and J.~F.~Gunion,
  %``Using decay angle correlations to detect CP violation in the neutral Higgs sector,''
  Phys.\ Lett.\ B {\bf 350} (1995) 218
  doi:10.1016/0370-2693(95)00369-V
  [hep-ph/9501339].
  %%CITATION = doi:10.1016/0370-2693(95)00369-V;%%
  %118 citations counted in INSPIRE as of 21 Nov 2016

%\cite{Takubo:2010tc}
\bibitem{Takubo:2010tc}
  Y.~Takubo, R.~N.~Hodgkinson, K.~Ikematsu, K.~Fujii, N.~Okada and H.~Yamamoto,
  %``Measuring anomalous couplings in $H \to WW^*$ decays at the International Linear Collider,''
  Phys.\ Rev.\ D {\bf 88} (2013) no.1,  013010
  doi:10.1103/PhysRevD.88.013010
  [arXiv:1011.5805 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.88.013010;%%
  %5 citations counted in INSPIRE as of 21 Nov 2016

\bibitem{Ogawa:2016}
T.~Ogawa, K.~Fujii and J.~Tian, "Study of anomalous VVH coupling at the ILC", 
talk at the LCWS15, paper in preparation.

%\cite{Anderson:2013afp}
\bibitem{Anderson:2013afp}
  I.~Anderson {\it et al.},
  %``Constraining anomalous HVV interactions at proton and lepton colliders,''
  Phys.\ Rev.\ D {\bf 89} (2014) no.3,  035007
  doi:10.1103/PhysRevD.89.035007
  [arXiv:1309.4819 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.89.035007;%%
  %69 citations counted in INSPIRE as of 21 Nov 2016

%\cite{Heister:2001uh}
\bibitem{Heister:2001uh}
  A.~Heister {\it et al.} [ALEPH Collaboration],
  %``Measurement of the tau polarization at LEP,''
  Eur.\ Phys.\ J.\ C {\bf 20} (2001) 401
  doi:10.1007/s100520100689
  [hep-ex/0104038].
  %%CITATION = doi:10.1007/s100520100689;%%
  %36 citations counted in INSPIRE as of 21 Nov 2016
  
%\cite{Desch:2003mw}
\bibitem{Desch:2003mw}
  K.~Desch, Z.~Was and M.~Worek,
  %``Measuring the Higgs boson parity at a linear collider using the tau impact parameter and tau ---> rho nu decay,''
  Eur.\ Phys.\ J.\ C {\bf 29} (2003) 491
  doi:10.1140/epjc/s2003-01231-4
  [hep-ph/0302046].
  %%CITATION = doi:10.1140/epjc/s2003-01231-4;%%
  %39 citations counted in INSPIRE as of 21 Nov 2016

%\cite{Rouge:2005iy}
\bibitem{Rouge:2005iy}
  A.~Rouge,
  %``CP violation in a light Higgs boson decay from tau-spin correlations at a linear collider,''
  Phys.\ Lett.\ B {\bf 619} (2005) 43
  doi:10.1016/j.physletb.2005.05.076
  [hep-ex/0505014].
  %%CITATION = doi:10.1016/j.physletb.2005.05.076;%%
  %13 citations counted in INSPIRE as of 21 Nov 2016
  
%\cite{Jeans:2015vaa}
\bibitem{Jeans:2015vaa}
  D.~Jeans,
  %``Tau lepton reconstruction at collider experiments using impact parameters,''
  Nucl.\ Instrum.\ Meth.\ A {\bf 810} (2016) 51
  doi:10.1016/j.nima.2015.11.030
  [arXiv:1507.01700 [hep-ex]].
  %%CITATION = doi:10.1016/j.nima.2015.11.030;%%
  %3 citations counted in INSPIRE as of 21 Nov 2016

%\cite{Harnik:2013aja}
\bibitem{Harnik:2013aja}
  R.~Harnik, A.~Martin, T.~Okui, R.~Primulando and F.~Yu,
  %``Measuring CP violation in $h \to \tau^+ \tau^-$ at colliders,''
  Phys.\ Rev.\ D {\bf 88} (2013) no.7,  076009
  doi:10.1103/PhysRevD.88.076009
  [arXiv:1308.1094 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.88.076009;%%
  %34 citations counted in INSPIRE as of 21 Nov 2016

\bibitem{Jeans:2016}
 D.~Jeans, "Measuring the CP state of tau lepton pairs
2 from Higgs decay at the ILC", paper in preparation.
  
%\cite{Godbole:2011hw}
\bibitem{Godbole:2011hw}
  R.~M.~Godbole, C.~Hangst, M.~Muhlleitner, S.~D.~Rindani and P.~Sharma,
  %``Model-independent analysis of Higgs spin and CP properties in the process $e^+ e^- \to t \bar t \Phi$,''
  Eur.\ Phys.\ J.\ C {\bf 71} (2011) 1681
  doi:10.1140/epjc/s10052-011-1681-7
  [arXiv:1103.5404 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-011-1681-7;%%
  %26 citations counted in INSPIRE as of 21 Nov 2016
  
%\cite{Hagiwara:2016rdv}
\bibitem{Hagiwara:2016rdv}
  K.~Hagiwara, K.~Ma and H.~Yokoya,
  %``Probing CP violation in $e^{+}e^{-}$ production of the Higgs boson and toponia,''
  JHEP {\bf 1606} (2016) 048
  doi:10.1007/JHEP06(2016)048
  [arXiv:1602.00684 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP06(2016)048;%%
  %2 citations counted in INSPIRE as of 21 Nov 2016  
  
%\cite{Asner:2013psa}
\bibitem{Asner:2013psa}
  D.~M.~Asner {\it et al.},
  %``ILC Higgs White Paper,''
  arXiv:1310.0763 [hep-ph].
  %%CITATION = ARXIV:1310.0763;%%
  %196 citations counted in INSPIRE as of 21 Nov 2016  

\bibitem{Baer:2013yha}
  H.~Baer, V.~Barger, P.~Huang, D.~Mickelson, A.~Mustafayev, W.~Sreethawong and X.~Tata,
  %``Same sign diboson signature from supersymmetry models with light higgsinos at the LHC,''
  Phys.\ Rev.\ Lett.\  {\bf 110} (2013) no.15,  151801
  doi:10.1103/PhysRevLett.110.151801
  [arXiv:1302.5816 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.110.151801;%%
  %42 citations counted in INSPIRE as of 22 Nov 2016

\bibitem{Han:2014kaa}
  Z.~Han, G.~D.~Kribs, A.~Martin and A.~Menon,
  %``Hunting quasidegenerate Higgsinos,''
  Phys.\ Rev.\ D {\bf 89} (2014) no.7,  075007
  doi:10.1103/PhysRevD.89.075007
  [arXiv:1401.1235 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.89.075007;%%
  %67 citations counted in INSPIRE as of 22 Nov 2016

\bibitem{Baer:2014kya}
  H.~Baer, A.~Mustafayev and X.~Tata,
  %``Monojet plus soft dilepton signal from light higgsino pair production at LHC14,''
  Phys.\ Rev.\ D {\bf 90} (2014) no.11,  115007
  doi:10.1103/PhysRevD.90.115007
  [arXiv:1409.7058 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.90.115007;%%
  %43 citations counted in INSPIRE as of 22 Nov 2016
  
\bibitem{Heinemeyer:2013dia}
  S.~Heinemeyer, W.~Hollik, G.~Weiglein and L.~Zeune,
  JHEP {\bf 1312} (2013) 084
  [arXiv:1311.1663 [hep-ph]].
  %%CITATION = ARXIV:1311.1663;%%
  
\bibitem{Heinemeyer:2007bw}
  S.~Heinemeyer, W.~Hollik, A.~M.~Weber and G.~Weiglein,
  JHEP {\bf 0804} (2008) 039
  [arXiv:0710.2972 [hep-ph]].
  %%CITATION = ARXIV:0710.2972;%%
 
\bibitem{CMS:pas-hig-16-007}
CMS Collaboration, ``Summary results of high mass BSM Higgs searches using CMS run-I data ,''  CMS-PAS-HIG-16-007, \url{https://cds.cern.ch/record/2142432}. 

\bibitem{bib:atlas_higgsself_bbgg}
ATLAS Collaboration, ``Prospects for measuring Higgs pair production in the channel $H(\to \gamma\gamma)H(\to b\bar{b})$ using the ATLAS detector at the HL-LHC,'' ATLAS-PHYS-PUB-2014-019 (2014), \url{http://cds.cern.ch/record/1956733}.

\bibitem{bib:atlas_higgsself_bbtt}
ATLAS Collaboration, ``Higgs pair production in the $H(\to \tau\tau)H(\to b\bar{b})$ channel at the High-Luminosity LHC,'' ATLAS-PHYS-PUB-2015-046 (2015), \url{http://cds.cern.ch/record/2065974}.

\bibitem{bib:cms_higgsself}
CMS Collaboration, ``Technical Proposal for the Phase-II Upgrade of the Compact Muon Solenoid,'' CERN-LHCC-2015-010 (2015), \url{http://cds.cern.ch/record/2020886}.

%%%Begin citations RP

\bibitem{Grojean:2013qca}
C.~Grojean, O.~Matsedonskyi, and G.~Panico, ``{Light top partners and precision
  physics}''
\href{http://arxiv.org/abs/1306.4655}{{\tt arXiv:1306.4655 [hep-ph]}}.
%%CITATION = ARXIV:1306.4655;%%.

\bibitem{Agashe:2013hma}
{\bf Top Quark Working Group}, K.~Agashe {\em et al.}, ``{Working Group Report:
  Top Quark}'' in {\em {Proceedings, Community Summer Study 2013: Snowmass on
  the Mississippi (CSS2013): Minneapolis, MN, USA, July 29-August 6, 2013}}.
\newblock 2013.
\newblock \href{http://arxiv.org/abs/1311.2028}{{\tt arXiv:1311.2028
  [hep-ph]}}.
\newblock
\url{https://inspirehep.net/record/1263763/files/arXiv:1311.2028.pdf}.
\newblock
%%CITATION = ARXIV:1311.2028;%%.

\bibitem{Vos:2016til}
M.~Vos {\em et al.}, ``{Top physics at high-energy lepton colliders}''
\href{http://arxiv.org/abs/1604.08122}{{\tt arXiv:1604.08122 [hep-ex]}}.
%%CITATION = ARXIV:1604.08122;%%.

\bibitem{Fujii:2015jha}
K.~Fujii {\em et al.}, ``{Physics Case for the International Linear Collider}''
\href{http://arxiv.org/abs/1506.05992}{{\tt arXiv:1506.05992 [hep-ex]}}.
%%CITATION = ARXIV:1506.05992;%%.

\bibitem{Barklow:2015tja}
T.~Barklow, J.~Brau, K.~Fujii, J.~Gao, J.~List, N.~Walker, and K.~Yokoya,
  ``{ILC Operating Scenarios}''
\href{http://arxiv.org/abs/1506.07830}{{\tt arXiv:1506.07830 [hep-ex]}}.
%%CITATION = ARXIV:1506.07830;%%.

\bibitem{Senaha:2013fva}
E.~Senaha, ``{Overview of Electroweak Baryogenesis}'' in {\em {Proceedings, 1st
  Toyama International Workshop on Higgs as a Probe of New Physics 2013
  (HPNP2013): Toyama, Japan, February 13-16, 2013}}.
\newblock 2013.
\newblock \href{http://arxiv.org/abs/1305.1563}{{\tt arXiv:1305.1563
  [hep-ph]}}.
\newblock
\url{http://www.slac.stanford.edu/econf/C130213.1/pdfs/senaha.pdf}.
\newblock
%%CITATION = ARXIV:1305.1563;%%.

\bibitem{Godbole:2011hw}
R.~M. Godbole, C.~Hangst, M.~Muhlleitner, S.~D. Rindani, and P.~Sharma,
  ``{Model-independent analysis of Higgs spin and CP properties in the process
  $e^+ e^- \to t \bar t \Phi$}''
  \href{http://dx.doi.org/10.1140/epjc/s10052-011-1681-7}{{\em Eur. Phys. J.}
  {\bf C71} (2011)  1681},
\href{http://arxiv.org/abs/1103.5404}{{\tt arXiv:1103.5404 [hep-ph]}}.
%%CITATION = ARXIV:1103.5404;%%.

\bibitem{Seidel:2013sqa}
K.~Seidel, F.~Simon, M.~Tesar, and S.~Poss, ``{Top quark mass measurements at
  and above threshold at CLIC}'' {\em arXiv:1303.3758 [hep-ex]} (2013)  ,
\href{http://arxiv.org/abs/1303.3758}{{\tt arXiv:1303.3758 [hep-ex]}}.
%%CITATION = ARXIV:1303.3758;%%.

\bibitem{Beneke:2015kwa}
M.~Beneke, Y.~Kiyo, P.~Marquard, A.~Penin, J.~Piclum, and M.~Steinhauser,
  ``{Next-to-Next-to-Next-to-Leading Order QCD Prediction for the Top Antitop
  $S$-Wave Pair Production Cross Section Near Threshold in $e^+e^-$
  Annihilation}'' \href{http://dx.doi.org/10.1103/PhysRevLett.115.192001}{{\em
  Phys. Rev. Lett.} {\bf 115} (2015) no.~19, 192001},
\href{http://arxiv.org/abs/1506.06864}{{\tt arXiv:1506.06864 [hep-ph]}}.
%%CITATION = ARXIV:1506.06864;%%.

\bibitem{Marquard:2015qpa}
P.~Marquard, A.~V. Smirnov, V.~A. Smirnov, and M.~Steinhauser, ``{Quark Mass
  Relations to Four-Loop Order in Perturbative QCD}''
  \href{http://dx.doi.org/10.1103/PhysRevLett.114.142002}{{\em Phys.Rev.Lett.}
  {\bf 114} (2015) no.~14, 142002},
\href{http://arxiv.org/abs/1502.01030}{{\tt arXiv:1502.01030 [hep-ph]}}.
%%CITATION = ARXIV:1502.01030;%%.

\bibitem{bib:panico-priv}
{G. Panico, A. Wulzer, private communication, Possible deviations of couplings
  in framework described in~\cite{Grojean:2013qca}}.

\bibitem{Berger:2005ht}
C.~Berger, M.~Perelstein, and F.~Petriello, ``{Top quark properties in little
  Higgs models}''
\href{http://arxiv.org/abs/hep-ph/0512053}{{\tt arXiv:hep-ph/0512053
  [hep-ph]}}.
%%CITATION = HEP-PH/0512053;%%.

\bibitem{Carena:2006bn}
M.~S. Carena, E.~Ponton, J.~Santiago, and C.~E. Wagner, ``{Light Kaluza Klein
  States in Randall-Sundrum Models with Custodial SU(2)}''
  \href{http://dx.doi.org/10.1016/j.nuclphysb.2006.10.012}{{\em Nucl.Phys.}
  {\bf B759} (2006)  202--227},
\href{http://arxiv.org/abs/hep-ph/0607106}{{\tt arXiv:hep-ph/0607106
  [hep-ph]}}.
%%CITATION = HEP-PH/0607106;%%.

\bibitem{Pomarol:2008bh}
A.~Pomarol and J.~Serra, ``{Top Quark Compositeness: Feasibility and
  Implications}'' \href{http://dx.doi.org/10.1103/PhysRevD.78.074026}{{\em
  Phys.Rev.} {\bf D78} (2008)  074026},
\href{http://arxiv.org/abs/0806.3247}{{\tt arXiv:0806.3247 [hep-ph]}}.
%%CITATION = ARXIV:0806.3247;%%.

\bibitem{Cui:2010ds}
Y.~Cui, T.~Gherghetta, and J.~Stokes, ``{Fermion Masses in Emergent Electroweak
  Symmetry Breaking}'' \href{http://dx.doi.org/10.1007/JHEP12(2010)075}{{\em
  JHEP} {\bf 1012} (2010)  075},
\href{http://arxiv.org/abs/1006.3322}{{\tt arXiv:1006.3322 [hep-ph]}}.
%%CITATION = ARXIV:1006.3322;%%.

\bibitem{Barducci:2015aoa}
D.~Barducci, S.~De~Curtis, S.~Moretti, and G.~M. Pruna, ``{Top pair production
  at a future $e^+e^-$ machine in a composite Higgs scenario}''
\href{http://arxiv.org/abs/1504.05407}{{\tt arXiv:1504.05407 [hep-ph]}}.
%%CITATION = ARXIV:1504.05407;%%.

\bibitem{Djouadi:2006rk}
A.~Djouadi, G.~Moreau, and F.~Richard, ``{Resolving the A(FB)**b puzzle in an
  extra dimensional model with an extended gauge structure}''
  \href{http://dx.doi.org/10.1016/j.nuclphysb.2007.03.019}{{\em Nucl.Phys.}
  {\bf B773} (2007)  43--64},
\href{http://arxiv.org/abs/hep-ph/0610173}{{\tt arXiv:hep-ph/0610173
  [hep-ph]}}.
%%CITATION = HEP-PH/0610173;%%.

\bibitem{Richard:2014upa}
F.~Richard, ``{Present and future constraints on top EW couplings}''
\href{http://arxiv.org/abs/1403.2893}{{\tt arXiv:1403.2893 [hep-ph]}}.
%%CITATION = ARXIV:1403.2893;%%.

\bibitem{Amjad:2013tlv}
M.~Amjad, M.~Boronat, T.~Frisson, I.~Garcia, R.~Poschl, {\em et al.}, ``{A
  precise determination of top quark electro-weak couplings at the ILC
  operating at $\sqrt{s}=500$ GeV}''
\href{http://arxiv.org/abs/1307.8102}{{\tt arXiv:1307.8102 [hep-ex]}}.
%%CITATION = ARXIV:1307.8102;%%.

\bibitem{Amjad:2015mma}
M.~S. Amjad {\em et al.}, ``{A precise characterisation of the top quark
  electro-weak vertices at the ILC}''
  \href{http://dx.doi.org/10.1140/epjc/s10052-015-3746-5}{{\em accepted by
  European Journal of Physics C} (2015)  },
\href{http://arxiv.org/abs/1505.06020}{{\tt arXiv:1505.06020 [hep-ex]}}.
%%CITATION = ARXIV:1505.06020;%%.

\bibitem{Baur:2004uw}
U.~Baur, A.~Juste, L.~Orr, and D.~Rainwater, ``{Probing electroweak top quark
  couplings at hadron colliders}''
  \href{http://dx.doi.org/10.1103/PhysRevD.71.054013}{{\em Phys.Rev.} {\bf D71}
  (2005)  054013},
\href{http://arxiv.org/abs/hep-ph/0412021}{{\tt arXiv:hep-ph/0412021
  [hep-ph]}}.
%%CITATION = HEP-PH/0412021;%%.

\bibitem{Baur:2005wi}
U.~Baur, A.~Juste, D.~Rainwater, and L.~Orr, ``{Improved measurement of $ttZ$
  couplings at the CERN LHC}''
  \href{http://dx.doi.org/10.1103/PhysRevD.73.034016}{{\em Phys.Rev.} {\bf D73}
  (2006)  034016},
\href{http://arxiv.org/abs/hep-ph/0512262}{{\tt arXiv:hep-ph/0512262
  [hep-ph]}}.
%%CITATION = HEP-PH/0512262;%%.

\bibitem{Khachatryan:2015sha}
{\bf CMS}, V.~Khachatryan {\em et al.}, ``{Observation of top quark pairs
  produced in association with a vector boson in pp collisions at sqrt(s) = 8
  TeV}''
\href{http://arxiv.org/abs/1510.01131}{{\tt arXiv:1510.01131 [hep-ex]}}.
%%CITATION = ARXIV:1510.01131;%%.

\bibitem{Khiem:2015ofa}
P.~Khiem, E.~Kou, Y.~Kurihara, and F.~L. Diberder, ``{Probing New Physics using
  top quark polarization in the $e^+ e^- \rightarrow t \bar{t}$ process at
  future Linear Colliders}''
\href{http://arxiv.org/abs/1503.04247}{{\tt arXiv:1503.04247 [hep-ph]}}.
%%CITATION = ARXIV:1503.04247;%%.

\bibitem{Lees:2012xj}
{\bf BaBar}, J.~P. Lees {\em et al.}, ``{Evidence for an excess of $\bar{B} \to
  D^{(*)} \tau^-\bar{\nu}_\tau$ decays}''
  \href{http://dx.doi.org/10.1103/PhysRevLett.109.101802}{{\em Phys. Rev.
  Lett.} {\bf 109} (2012)  101802},
\href{http://arxiv.org/abs/1205.5442}{{\tt arXiv:1205.5442 [hep-ex]}}.
%%CITATION = ARXIV:1205.5442;%%.

\bibitem{Fujii:2016raq}
{\bf LCC Physics Working Group}, K.~Fujii {\em et al.}, ``{Implications of the
  750 GeV gamma-gamma Resonance as a Case Study for the International Linear
  Collider}''
\href{http://arxiv.org/abs/1607.03829}{{\tt arXiv:1607.03829 [hep-ph]}}.
%%CITATION = ARXIV:1607.03829;%%.

\bibitem{Randall:1999ee}
L.~Randall and R.~Sundrum, ``{A Large mass hierarchy from a small extra
  dimension}'' \href{http://dx.doi.org/10.1103/PhysRevLett.83.3370}{{\em
  Phys.Rev.Lett.} {\bf 83} (1999)  3370--3373},
\href{http://arxiv.org/abs/hep-ph/9905221}{{\tt arXiv:hep-ph/9905221
  [hep-ph]}}.
%%CITATION = HEP-PH/9905221;%%.

\bibitem{Kakizaki:2015zva}
M.~Kakizaki, S.~Kanemura, M.~Kikuchi, T.~Matsui, and H.~Yokoya, ``{Indirect
  reach of heavy MSSM Higgs bosons by precision measurements at future lepton
  colliders}'' \href{http://dx.doi.org/10.1142/S0217751X15501924}{{\em Int. J.
  Mod. Phys.} {\bf A30} (2015) no.~33, 1550192},
\href{http://arxiv.org/abs/1505.03761}{{\tt arXiv:1505.03761 [hep-ph]}}.
%%CITATION = ARXIV:1505.03761;%%.

\bibitem{Aaboud:2016cre}
{\bf ATLAS}, M.~Aaboud {\em et al.}, ``{Search for Minimal Supersymmetric
  Standard Model Higgs bosons $H/A$ and for a $Z^{\prime}$ boson in the $\tau
  \tau$ final state produced in $pp$ collisions at $\sqrt{s}=13$ TeV with the
  ATLAS Detector}''
  \href{http://dx.doi.org/10.1140/epjc/s10052-016-4400-6}{{\em Eur. Phys. J.}
  {\bf C76} (2016) no.~11, 585},
\href{http://arxiv.org/abs/1608.00890}{{\tt arXiv:1608.00890 [hep-ex]}}.
%%CITATION = ARXIV:1608.00890;%%.

\bibitem{Malm:2014gha}
R.~Malm, M.~Neubert, and C.~Schmell, ``{Higgs Couplings and Phenomenology in a
  Warped Extra Dimension}''
  \href{http://dx.doi.org/10.1007/JHEP02(2015)008}{{\em JHEP} {\bf 02} (2015)
  008},
\href{http://arxiv.org/abs/1408.4456}{{\tt arXiv:1408.4456 [hep-ph]}}.
%%CITATION = ARXIV:1408.4456;%%.

\bibitem{Cerrito:2016qig}
L.~Cerrito, D.~Millar, S.~Moretti, and F.~Span{\`o}, ``{Discovering and
  profiling Z' bosons using asymmetry observables in top pair production with
  the lepton-plus-jets final state at the LHC}''
\href{http://arxiv.org/abs/1609.05540}{{\tt arXiv:1609.05540 [hep-ph]}}.
%%CITATION = ARXIV:1609.05540;%%.

\bibitem{Accomando:2010fz}
E.~Accomando, A.~Belyaev, L.~Fedeli, S.~F. King, and
  C.~Shepherd-Themistocleous, ``{Z' physics with early LHC data}''
  \href{http://dx.doi.org/10.1103/PhysRevD.83.075012}{{\em Phys. Rev.} {\bf
  D83} (2011)  075012},
\href{http://arxiv.org/abs/1010.6058}{{\tt arXiv:1010.6058 [hep-ph]}}.
%%CITATION = ARXIV:1010.6058;%%.

\bibitem{ATLAS-CONF-2016-045}
{\bf ATLAS Collaboration}, ``{Search for new high-mass resonances in the
  dilepton final state using proton-proton collisions at $\sqrt{s}$ = 13 TeV
  with the ATLAS detector}'' Tech. Rep. ATLAS-CONF-2016-045, CERN, Geneva, Aug,
  2016.
\newblock \url{http://cds.cern.ch/record/2206127}.

%End citations RP

\end{thebibliography}

